Fixing Bias in Reconstruction-based Anomaly Detection with Lipschitz Discriminators

Anomaly detection is of great interest in fields where abnormalities need to be identified and corrected (e.g., medicine and finance). Deep learning methods for this task often rely on autoencoder reconstruction error, sometimes in conjunction with other errors. We show that this approach exhibits intrinsic biases that lead to undesirable results. Reconstruction-based methods are sensitive to training-data outliers and simple-to-reconstruct points. Instead, we introduce a new unsupervised Lipschitz anomaly discriminator that does not suffer from these biases. Our anomaly discriminator is trained, similar to the ones used in GANs, to detect the difference between the training data and corruptions of the training data. We show that this procedure successfully detects unseen anomalies with guarantees on those that have a certain Wasserstein distance from the data or corrupted training set. These additions allow us to show improved performance on MNIST, CIFAR10, and health record data.

==> figures/generalization_dispersion.tex <==
\begin{figure}[ht]
    \begin{center}
    \includegraphics[width=0.8\linewidth]{figures/generalization_dispersion.png}
    \end{center}
    \caption{Plots the AUC on CIFAR10 classes vs. the dispersion, measured by the average distance to the mean image in that class. Autoencoders tend to work better on more concentrated classes.}
    \vspace{-5mm}
    \label{fig:generalization-dispersion}
\end{figure}

==> figures/mnist_by_digit.tex <==
\begin{figure*}[ht]
    \begin{center}
    \includegraphics[width=0.8\linewidth]{figures/mnist_by_digit_v1.png}
    \end{center}
    \caption{Shows the AUC across digits of all models with 95\% confidence error bars over 3 seeds. Some digits are more difficult than others Our model does particularly well on the digit 8, outperformaing all other models by a significant margin on all training set corruptions tested.}
    \label{fig:comparison}
\end{figure*}

==> figures/mnist_standard.tex <==
\begin{figure*}[ht]
    \begin{center}
    \includegraphics[width=0.5 \linewidth]{figures/mnist_standard_v3.png}
    \end{center}
    \caption{Shows the area under the receiver operator characteristic curve (auc) of various anomaly detection models with varying levels of training set contamination on MNIST data. For contamination $>1\%$ our model (LAD) outperforms all other deep models.}
    \label{fig:standard}
\end{figure*}


==> figures/moons/moons.tex <==
\begin{figure}[ht]
\centering
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/moons/input.png}
  \caption{Input Data}
  \label{fig:moons:sfig1}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/moons/plot_ae.png}
  \caption{Reconstruction error as score}
  \label{fig:moons:sfig2}
\end{subfigure}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/moons/plot.png}
  \caption{Our discriminator-based score}
  \label{fig:moons:sfig3}
\end{subfigure}

\caption{(a) training data (b) autoencoder reconstruction score (c) LAD anomaly score (Red = more normal, blue = more anomalous). Reconstruction is a poor proxy for data density, particularly when far from the data.}
\vspace{-5mm}
%\caption{Depicts the anomaly score over the plane of an autoencoder reconstruction model and our Lipschitz anomaly discriminator trained on \texttt{sklearn.datasets.make\_moons} data (Red = more normal, blue = more anomalous). Reconstruction is a poor proxy for data density.}
\label{fig:moons}
\end{figure}

==> figures/prev_work.tex <==

\begin{table}
\begin{tabular}{lrrrrr}
\toprule
& deep model & model based  & distance based    & reconstruction error score    & adversarial \\
\cite{pearson_lines_1901-2, wright_robust_2009}
&            & \checkmark   &                   & \checkmark & \\
\cite{schlegl_f-anogan_2019, ravanbakhsh_abnormal_2017}
& \checkmark & \checkmark  &                    & \checkmark                    & \checkmark \\
\cite{breunig_lof_2000, elomaa_fast_2002, zhao_anomaly_2009}
&            &              & \checkmark        &                               & \\
\cite{ravanbakhsh_abnormal_2017, schlegl_f-anogan_2019}
\bottomrule
\end{tabular}
\caption{Shows the anomaly rank of the black image in the MNIST test set of each digit trained on the training set for each digit. Since the black image is inherently easy to reconstruct, it receives a low anomaly score in reconstruction based models.}
\label{tab:prev-work}
\end{table}


==> sections/2_related_work.tex <==



% \noindent\paragraph{Reconstruction-based methods.}
% Many works use an information constrained model trained with reconstruction error assuming that outliers will be poorly reconstructed. In more recent work \cite{chalapathy_robust_2017, abati_latent_2019, perera_ocgan_2019} the authors add losses to constrain the latent space of an autoencoder to better limit the capacity, but these are still fundamentally based on reconstruction penalty. 
% Existing anomaly detectors built in the adversarial framework either compute reconstruction error in the latent space~\cite{schlegl_unsupervised_2017} or constrain the latent space of an autoencoder~\cite{sabokrou_adversarially_2018}. These methods still use reconstruction error as the main score. 

%There are a few ways discriminator losses have been incorporated in existing work, however they all ultimately rely on reconstruction error. The first is by training a GAN to learn the data manifold, the closest point in the manifold is found using back-propogation~\cite{schlegl_unsupervised_2017}, or additional machinery~\cite{zenati_efficient_2018} reconstruction error between the generated image and the test image~\cite{akcay_ganomaly_2018}, these methods do not perform as well as autoencoders when scoring whole images~\cite{sabokrou_adversarially_2018, di_mattia_survey_2019}, and may suffer from the same type of problems as we note in this paper on autoencoder based reconstruction scoring. Other work attempts to constrain the autoencoder embedding space such that it only represents only in-class points~\cite{perera_ocgan_2019} or conforms to a prior distribution~\cite{pidhorskyi_generative_2018}. This may remove some of the accurately reconstructed low-density interpolations, but may make it even more sensitive to outliers by increasing the volume of embedded space assigned to each sample in the training set.

%\paragraph{Support vector methods.} Support vector based methods attempt to separate the normal data from the anomalous space with either planes (OC-SVM)~\cite{scholkopf_estimating_2001} or hyperspheres (SVDD)~\cite{tax_support_2004}. One-class neural networks (OC-NN)~\cite{chalapathy_anomaly_2018} and deep support vector data description (DSVDD) in \cite{ruff_deep_2018} generalize these to use deep networks. These methods attempt to create an embedding space where standard OC-NN and SVDD can be applied. These generalizations do not perform as well as autoencoder based methods~\cite{pidhorskyi_generative_2018, perera_ocgan_2019}.

%\paragraph{Distance-based density estimation methods.} A relatively efficient way to estimate density is using nearest neighbor distances~\cite{knorr_distance-based_2000, ramaswamy_efcient_2000, zhao_anomaly_2009, elomaa_fast_2002}. We compare against the method in \cite{breunig_lof_2000} as one of the best performing methods over a wide variety of datasets~\cite{zimek_survey_2012,campos_evaluation_2016}. However, these methods require a $k$-nearest neighbor query, which requires at least $O(n \log n)$ time and at least $O(n)$ space~\cite{bentley_multidimensional_1975}. We instead use a model-based method that has complexity independent of dataset size. We adapt the distance based framework to high dimensions using the dual formulation of the Wasserstein distance. %To the best of our knowledge our work is the first to explore the benefits of adapting density based methods to neural network anomaly detection.

%Our method acts like a distance based method especially outside of the support of the distribution 

% Can we show that the LAD f* is equivalent to a distance based penalty outside of the convex hull?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Existing methods generally fall into two categories model or distance based. Within model based anomaly detection we can further make the distinction between methods that score test points based on reconstruction, and those that attempt to directly estimate the data density. 

%Two examples of model based algorithms are one-class support vector machines (OC-SVM), which learns a half-space separating the data from the origin, and support vector data description (SVDD), which learns the smallest hypersphere surround the data~\cite{scholkopf_estimating_2001, tax_support_2004}. Other methods based on truncated PCA or its variants use reconstruction error on a truncated basis of the data~\cite{pearson_lines_1901-2, wright_robust_2009}. The main drawback to these methods is their poor performance in high dimensional datasets. In recent years, many deep methods attempt to generalize these objectives to neural networks as a way of overcoming this problem in the image domain. 

%Autoencoder based models use an autoencoder or variant to estimate density by either using the learned embedding and using a linear model~\cite{andrews_detecting_2016,erfani_high-dimensional_2016} or by taking the reconstruction loss of a test point~\cite{hawkins_outlier_2002, sakurada_anomaly_2014}. A few works take a step further and generalize objectives used in linear methods to the autoencoder setting. \citet{chalapathy_robust_2017} generalize the robust PCA objective. \citet{ruff_deep_2018} generalize the SVDD objective. \citet{chalapathy_anomaly_2018} generalize the OC-SVM objective. \citet{abati_latent_2019} add an autoregressive loss to the reconstruction loss. For a recent survey see~\cite{chalapathy_deep_2019}. However, in this work we show that reconstruction error is not a good proxy for data density (see Figure~\ref{fig:moons}) and is not robust, as some datapoints are less difficult to reconstruct than others (See Table~\ref{tab:black-image}). Furthermore, our model is the first that can be thought of generalizing distance based anomaly detection to neural networks.

%A number of generative adversarial network (GAN) based methods have been suggested for detecting anomalous areas within a test image, but can be used for our task. \citet{schlegl_f-anogan_2019} uses a reconstruction error based on the Bi-GAN~\cite{donahue_adversarial_2016} architecture. \citet{ravanbakhsh_abnormal_2017} also uses reconstruction error for anomaly detection in videos. \citet{pidhorskyi_generative_2018,perera_ocgan_2019} use adversarial autoencoder~\cite{makhzani_adversarial_2015-1} based approaches and a probabilistic interpretation of the latent space. However, these methods are designed to detect anomalies within test points by highlighting anomalous regions of a test image, and as such are not optimized for point-wise anomaly detection (See Table~\ref{tab:large_comparison}).

%Out of the GAN methods, \citet{sabokrou_adversarially_2018} is the most similar method to our work, as they also uses the discriminator of a GAN as their anomaly scoring function. Their method could be restated as training a denoising convolutional autoencoder (DCAE)~\cite{vincent_stacked_2010-1} followed by a discriminator loss between its output (fake) and its input (real). We note three advantages of our method over \cite{sabokrou_adversarially_2018}. (1) We do not need to train a generator network avoiding the many difficulties in training of adversarial networks \cite{salimans_improved_2016}. (2) We use a Lipschitz discriminator guaranteeing that points that are close together receive similar scores. (3) We do not use a reconstruction based loss, which biases nominal points towards those that are easy to reconstruct, and not those that are close to training points. By using a Lipschitz constrained network we use a distance interpretation unlike any previous deep method. 

%More traditional non-network based methods for anomaly detection often use a distance based estimation of density. These methods use a K-NN approach for determining anomalies and have been shown to work well in a wide variety of settings. These methods attempt to estimate the local density of a point either relative to its neighbors as in~\cite{breunig_lof_2000} or to the entire dataset as in ~\cite{zhao_anomaly_2009}. These methods have been shown to perform quite well on a variety of tasks~\cite{zimek_survey_2012,campos_evaluation_2016}. However, these methods require a $k$-nearest neighbor query, which requires at least $O(n \log n)$ time and at least $O(n)$ space using spatial indexing structures~\cite{bentley_multidimensional_1975}. In this work, we generalize a distance based method to the network domain showing both theoretical and empirical benefits over existing deep anomaly detection methods.





==> sections/3_biases_in_reconstruction.tex <==
\section{Biases in Reconstruction-based Methods}
\label{sec:bias}
We focus on biases in reconstruction-based methods because the best performing methods are based on autoencoders with a few tweaks~\cite{perera_ocgan_2019, abati_latent_2019}.

\paragraph{C1. Sensitivity to outliers.} As a loss function, mean-squared error tends to focus more on outlier points (points with poor reconstruction) due to the squared term ~\cite{bermejo_oriented_2001}. This is a problem when considering outliers contaminating the normal training data, as the autoencoder will learn to reconstruct these points well, even if they are far away from the rest of the data. In section~\ref{sec:exp:contamination}, we show how contaminating the training set with a small amount of anomalous points rapidly decreases the effectiveness of autoencoder-based anomaly detection. This effect leads to the systematic underestimation of anomaly score using reconstruction error near single points in low density regions of the input space.

\paragraph{C2. Behavior of autoencoders in the interior.} 
Recent work shows that neural networks exist in an interpolating regime~\cite{belkin_reconciling_2019, belkin_two_2019, nakkiran_deep_2019}. When the number of parameters is large, the generalization error continues to decrease even after the training error has hit zero~\cite{hastie_surprises_2019}. Work on the interpolation regime helps us to further understand the biases of autoencoders. This leads us to the hypothesis that autoencoders interpolate too well for anomaly detection and may reconstruct points within the data well, even in low or no density regions. In Figure~\ref{fig:circle}, while there is no density in the center of the ring, the autoencoder learns to reconstruct many interpolated points in the center of the ring well. In Table~\ref{tab:black-image-short} we show how autoencoders do not score the black image as an anomaly when trained on MNIST.


It is interesting to consider the behavior of an autoencoder with one overparameterized layer where the number of samples $n$ is less than the width $w$. We consider the minimum norm solution for the autoencoding problem. This is well known to correspond to a projection onto the span of the data~\cite{engl_regularization_1996}. A corollary is that in this setting, \textit{any point in the span of the training data has zero training error}. \citet{radhakrishnan_memorization_2019} showed that this also holds for a non-linear extension. Since points interior to the convex hull are a subset of the span of the training data, all points lying within the convex hull also have zero reconstruction error. This suggests that a MSE trained autoencoder may be explicitly biased towards reconstructing points in the hull of the data well, and may have trouble detecting outliers within the hull of the data. Our method is explicitly designed to be able to detect these types of outliers.
%\begin{prop} For an overparamterized single layer linear autoencoder $y=Ax$ trained on $U=\{u_0, \ldots, \u_n\}$ with gradient descent initialized at zero the reconstruction error at $x$ can be written as:
%RE(x) = 

% A = Q^T I Q for n points in $U$ thus it is the projection onto U. 
%\end{prop}
 %In the MNIST dataset, this is not much of an issue as \todo{WHAT PERCENT RY:more than 25\%} of test images are outside of the convex hull of the training images. However, there are many reasonable datasets where this is not the case.

Given that autoencoders are known to reconstruct interpolations well, it is not surprising that they also seem to reconstruct images close to the mean image well (Fig.~\ref{fig:cifar}). An autoencoder trained on the `car' images in CIFAR reconstructs images that are close to the mean car (Fig. ~\ref{fig:cifar:sfig3}) better than those that are real cars, but far from the mean. We notice that the CIFAR classes with low dispersion are also the ones where autoencoders perform best (Fig.~\ref{fig:generalization-dispersion}). LAD has the opposite bias.

\input{figures/generalization_dispersion.tex}

%\subsection{Behavior of autoencoders outside the convex hull.}

%Our experiments on MNIST show that the farther a testing image is from the convex hull of training data, it is more likely to have a high anomaly score, too (Fig.~\ref{fig:out-convex}). This aligns with the arguments we have discussed so far. Data outside the convex hull cannot be reconstructed by interpolating between the training examples. Instead, closeness to the convex hull is the main discriminator.

%This relationship is observed before in the general literature for anomaly detection, e.g., \cite{}. However, it is not studied for deep learning models. 
%\%todo{Roozbeh}

%\cite{haffner2002escaping}

%\cite{vincent2002k}
%\todo{
%\begin{enumerate}
%    \item Can we show that points far from the convex hull have higher variance in reconstruction score by autoencoders? This suggests autoencoders are ``less sure'' about points that are far from training examples.
%    \item In a 2d example, show how adding a single example far from the data changes the score dramatically around it. 
%    \item Prove that the reconstruction behavior of a 1 layer autoencoder is IDK
%    \item How can we explain differing performance on different classes of images for different models?
%\end{enumerate}
%}


%\subsection{Training an autoencoder on a single image.} We consider training an autoencoder on a single image. This has been explored before in autoencoders through visualization of the reconstructions~\cite{zhang_identity_2020}, but we wanted to see the quality of reconstructions. We found that the digit `1' is particularly easy to reconstruct for a convolutional autoencoder, even after correcting by the distance to the training image. In Figure~\ref{fig:reconstruction-bias-short}, we can see how even trained on a single image, a convolutional autoencoder has significant biases towards which class of image are easy to reconstruct. This holds regardless of which class the single image comes from (see Figure~\ref{fig:reconstruction-bias}).

%\input{figures/reconstruction_bias_short.tex}

==> sections/old_new_theory.tex <==
\paragraph{Theoretical Results.} To address the robustness to corruption of the training set theoretically, suppose our training set is corrupted with a fraction $\gamma > 0$ of anomalous datapoints, then we show that our method should still effectively distinguish between nominal and anomalous datapoints. 

Because we are training the discriminator to maximize the difference between the nominal and corrupted points if our corruption process follows the distribution of anomalies (i.e., $\widehat{P_a} = P_a$) then the change in the difference between the nominal and anomalous points is bounded from below.

\begin{prop} 
\label{prop:robustness}
Let $f^{(A,B)}$ denote the optimal solution to $\max_{\|f\|_L \le 1} \mathbb{E}_{x \sim A} f(x) - \mathbb{E}_{x \sim B} f(x)$, and in particular let $f^* = f^{(P_n, P_a)}$ and $f^{**} = f^{((1 - \gamma) P_n + \gamma P_a, P_a)}$. Then, under the same conditions as Prop.~\ref{prop:threshold},
\begin{align*}
\bigl |\mathbb{E}_{x \sim P_n} [f^*(x) - f^{**}(x)] + \mathbb{E}_{x \sim P_a} [f^{**}(x) - f^{*}(x)] \bigr | \\
%\le \frac{\gamma}{1 - \gamma} W(P_n, P_a)
\le \frac{1}{1 - \gamma} W(P_n, (1-\gamma) P_n + \gamma P_a)
\end{align*}
\end{prop}
See Appendix~\ref{sec:proofs} for proof. This result can be thought of bounding the increase of score on the anomaly points and the decrease of score on the normal points (or vice versa) when the training set is corrupted by the addition of anomalies to it, where $0 \leq \gamma \leq 1$ represents the amount corruption. When the training set is corrupted by a small amount the anomaly scoring function does not change too much in expectation. For a score based on autoencoder reconstruction error a single point can affect the scoring function an arbitrary amount. For example, take an anomaly distribution that is a dirac at one point which is easily reconstructable, e.g. the black image in MNIST. Then corrupting the training data with a single anomalous example can take the MSE to zero for the entire anomaly distribution. This is an adversarial case, however we find that this also occurs in practice.

Finally, we would like to bound the difference between the optimal discriminator function and the one learned by our estimate $\widehat{P_a}$ of the unknown true $P_a$. We note that this can be achieved directly from the triangle inequality over the Wasserstein distance. Indeed, since both $W(P_n, P_a) \le W(P_a, \widehat{P_a}) + W(\widehat{P_a},P_n)$ and $W(P_n, \widehat{P_a}) \le W(P_n, P_a) + W(P_a, \widehat{P_a})$, then 
\begin{align}
    \label{eq:stability}
    \bigl |W(P_n, P_a) - W(P_n, \widehat{P_a}) \bigr 
    |% &= \max\{W(P_n, P_a) - W(P_n, \widehat{P_a}), W(P_n, \widehat{P_a}) - W(P_n, P_a)\}  \\
    &\le W(P_a, \widehat{P_a})
\end{align}

We formalize this in our Proposition~\ref{prop:threshold}. Intuitively, points sufficiently far away from the data will have a higher anomaly score than any point in the data.

\begin{prop}
\label{prop:threshold}
Let $f^*$ be the optimal solution of $\sup_{\|f\|_L \le 1} \left( \mathbb{E}_{x \sim P_n} [f(x)] - \mathbb{E}_{y \sim P_a} [f(y)] \right)$, and let $\pi$ be the optimal coupling between $P_n$ and $P_a$, defined as the minimizer of $W(P_n, P_a) = \inf_{\pi \in \Pi(P_n, P_a)} \mathbb{E}_{(x,y) \sim \pi} [ \|x - y\| ]$ where $\Pi(P_n, P_a)$ is the set of joint distributions whose marginals are $P_n$ and $P_a$, respectively. If $P_n$ has a compact support $\mathcal{S}_n$ and $P_a$ has compact support $\mathcal{S}_a$, then there exists $C > 0$ such that $f^*(y) \leq C - \inf_{x \in \mathcal{S}_n}\{\|x - y\|\}$ for $P_a$-almost every $y$.
\end{prop}

\begin{cor}
\label{corr:threshold}
Under the conditions of Prop.~\ref{prop:threshold}, there exists $R > 0$ such that for $P_a$-almost every $y$, if $\inf_{x \in \mathcal{S}_n} \|y - x\| > R$ then $f^*(y) < f^*(x)$ for $P_n$-almost every $x$. 
\end{cor}

See Appendix~\ref{sec:proofs} for proof. For a single training example, this can be understood as a peak at the training example, with $f^*$ decaying with slope 1 in every direction from this point.

==> tables/avg_dist_to_mean.tex <==
\begin{table}
\centering
\scalebox{0.9}{
\begin{tabular}{lr}
\toprule
{} &  avg dist to mean \\
\midrule
plane &            746.52 \\
car   &            846.56 \\
bird  &            647.88 \\
cat   &            800.02 \\
deer  &            546.46 \\
dog   &            742.65 \\
frog  &            604.37 \\
horse &            725.76 \\
ship  &            661.08 \\
truck &            772.83 \\
\bottomrule
\end{tabular}
}
\caption{Average distance to mean image for CIFAR10 training sets.}
%Using distance based methods such as LOF also perform reasonably well, although not consistently across digits.
\label{tab:avg_dist_to_mean}
\end{table}

==> tables/black_image_table.tex <==
\begin{table*}
\centering
\scalebox{0.9}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Digit &      0 &      1 &      2 &      3 &      4 &      5 &      6 &      7 &      8 &      9 &   mean \\
\midrule

ALOCC~\cite{sabokrou_adversarially_2018}      &  0.351 &  0.015 &  0.199 &  0.194 &  0.204 &  0.216 &  0.164 &  0.121 &  0.160 &  0.060 &  0.168 \\
CAE~\cite{hawkins_outlier_2002}        &  0.017 &  0.395 &  0.010 &  0.001 &  0.014 &  0.001 &  0.053 &  0.083 &  0.091 &  0.002 &  0.067 \\
DCAE~\cite{vincent_stacked_2010-1}       &  0.001 &  0.149 &  0.001 &  0.001 &  0.008 &  0.001 &  0.001 &  0.001 &  0.299 &  0.126 &  0.059 \\
DSVDD~\cite{ruff_deep_2018}      &  0.757 &  0.480 &  0.136 &  0.368 &  0.917 &  0.273 &  0.847 &  0.571 &  0.627 &  0.736 &  0.571 \\
%AND~\cite{abati_latent_2019}        &  0.426 & 0.023 & 0.895 & 0.294 & 0.143 & 0.216 & 0.011 & 0.561 & 0.071 & 0.063 & 0.270 \\
%IF~\cite{liu_isolation-based_2012}         &  0.587 &  0.818 &  0.035 &  0.324 &  0.123 &  0.001 &  0.235 &  0.271 &  0.365 &  0.363 &  0.312 \\
LOF~\cite{breunig_lof_2000}        &  0.876 &  0.986 &  0.140 &  0.625 &  0.765 &  0.330 &  0.961 &  0.865 &  0.509 &  0.895 &  0.695 \\
OCSVM~\cite{scholkopf_estimating_2001}      &  0.916 &  0.977 &  0.355 &  0.498 &  0.668 &  0.259 &  0.803 &  0.863 &  0.553 &  0.873 &  0.677 \\
RCAE~\cite{chalapathy_robust_2017}       &  0.023 &  0.418 &  0.001 &  0.001 &  0.001 &  0.001 &  0.005 &  0.001 &  0.007 &  0.033 &  0.049 \\
LAD (ours) &  \textbf{1.000} &  \textbf{1.000} &  \textbf{1.000} &  \textbf{1.000} &  \textbf{1.000} & \textbf{1.000} &  \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
\bottomrule
\end{tabular}
}
\caption{Shows the mean anomaly rank of the black image in the nominal test data. Scores are in $[0,1]$, with 1 as the best. Scores are measured on the MNIST test set of each digit trained on the uncorrupted training set for each digit over 3 seeds. Since the black image is inherently easy to reconstruct, it receives a low anomaly score in reconstruction based models.}
%Using distance based methods such as LOF also perform reasonably well, although not consistently across digits.
\label{tab:black-image}
\end{table*}

==> tables/black_image_table_short.tex <==
\begin{table}
\centering
\scalebox{0.9}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 &       mean \\
\midrule
ALOCC~\cite{sabokrou_adversarially_2018}        &   0.168 \\
CAE~\cite{hawkins_outlier_2002}                 &   0.067 \\
DCAE~\cite{vincent_stacked_2010-1}              &  0.059 \\
DSVDD~\cite{ruff_deep_2018}                     &  0.571 \\
%AND~\cite{abati_latent_2019}        &   0.270 \\
IF~\cite{liu_isolation-based_2012}         &  0.312 \\
LOF~\cite{breunig_lof_2000}                 &   0.695 \\
OCSVM~\cite{scholkopf_estimating_2001}      &   0.677 \\
RCAE~\cite{chalapathy_robust_2017}       & 0.049 \\
LAD (ours) &  \textbf{1.000} \\
\bottomrule
\end{tabular}
}
\caption{Shows the mean anomaly rank of the black image in the nominal test data mean over all digits.}
\vspace{-5mm}
%Using distance based methods such as LOF also perform reasonably well, although not consistently across digits.
\label{tab:black-image-short}
\end{table}

==> tables/cifar_table_full.tex <==
\begin{table*}[ht]
\centering
\scalebox{0.85}{
\begin{tabular}{lrrrrrrrrrr|r}
\toprule
{} &  plane &  car &      bird &       cat &      deer &       dog &      frog &     horse &      ship &     truck &      mean \\
\midrule
ALOCC~\cite{sabokrou_adversarially_2018}    &  0.421 &  0.439 &  0.530 &  0.505 &  0.500 &  0.473 &  0.500 &  0.377 &  0.387 &  0.500 &  0.463 \\
AND~\cite{abati_latent_2019}                &  0.717 &  0.494 &  0.662 &. 0.527 &  0.736 &  0.504 &. 0.726 &  0.560 &  0.680 &  0.566 &. 0.617 \\
AnoGAN~\cite{schlegl_unsupervised_2017}     &  0.671 &  0.547 &  0.529 &  0.545 &  0.651 &  0.603 &  0.585 &  0.625 &  0.758 &  0.665 &  0.618 \\
CAE~\cite{hawkins_outlier_2002}             &  0.683 &  0.454 &  0.677 &  0.524 &  0.765 &  0.525 &  0.731 &  0.541 &  0.706 &  0.435 &  0.604 \\
DCAE~\cite{vincent_stacked_2010-1}          &  0.689 &  0.447 &  0.679 &  0.534 &  0.765 &  0.526 &  0.729 &  0.539 &  0.717 &  0.426 &  0.605 \\
DSVDD~\cite{ruff_deep_2018}                 &  0.518 &  0.656 &  0.528 &  0.530 &  0.565 &  0.568 &  0.587 &  0.565 &  0.540 &  0.650 &  0.571 \\
IF~\cite{liu_isolation-based_2012}          &  0.670 &  0.442 &  0.645 &  0.512 &  0.743 &  0.516 &  0.711 &  0.529 &  0.694 &  0.529 &  0.599 \\
LOF~\cite{breunig_lof_2000}                 &  0.661 &  0.440 &  0.649 &  0.506 &  0.688 &  0.511 &  0.692 &  0.518 &  0.685 &  0.405 &  0.575 \\
OCSVM~\cite{chen_one-class_2001}            &  0.684 &  0.456 &  0.674 &  0.509 &  0.749 &  0.502 &  0.699 &  0.501 &  0.670 &  0.453 &  0.590 \\
RCAE~\cite{chalapathy_robust_2017}          &  0.675 &  0.429 &  0.669 &  0.541 &  0.745 &  0.531 &  0.690 &  0.527 &  0.710 &  0.404 &  0.592 \\
LAD (ours)                                  &  0.597 &  0.663 &  0.411 &  0.531 &  0.362 &  0.561 &  0.409 &  0.592 &  0.777 &  0.744 &  0.565 \\
LAD + CAE (ours)                            &  0.723 &  0.497 &  0.652 &  0.538 &  0.725 &  0.544 &  0.714 &  0.565 &  0.763 &  0.529 &  0.635 \\


\bottomrule
\end{tabular}
}
%\vspace{-3mm}
\caption{AUC on representative CIFAR10 classes over 3 seeds with mean over all classes.}
%\vspace{-5mm}
\label{tab:cifar-corrupt}
\end{table*}

%OCGAN~\cite{perera_ocgan_2019} & \textbf{0.757} &0.531& 0.640& \textbf{0.620}& 0.723& \textbf{0.620}& 0.723& 0.575& \textbf{0.820}& 0.554& \textbf{0.657}\\

==> tables/full_table.tex <==
\begin{table*}
\scalebox{0.89}{
\begin{tabular}{lrrrrrrrrrr|r}
\toprule
 &      0 &      1 &      2 &      3 &      4 &      5 &      6 &      7 &      8 &      9 &   Mean \\
\midrule

LAD (ours)                                          &  0.984 &  0.992 &  0.920 &  0.917 &  0.921 &  0.871 &  0.971 &  0.942 &  0.928 &  0.945 &  0.939 \\
CAE                                                 &  0.996 &  0.999 &  0.946 &  0.940 &  0.971 &  0.945 &  0.992 &  0.979 &  0.901 &  0.985 &  0.965 \\
DCAE                                                &  0.997 &  \textbf{1.000} &  0.957 &  0.930 &  0.972 &  0.968 &  0.990 &  0.976 &  0.899 &  0.986 &  0.967 \\
RCAE~\cite{chalapathy_robust_2017}                  &  0.996 &  0.999 &  0.930 &  0.928 &  0.967 &  0.921 &  0.994 &  0.973 &  0.885 &  0.984 &  0.958 \\

DAE                                                 &  0.894 &  0.999 &  0.792 &  0.851 &  0.888 &  0.819 &  0.944 &  0.922 &  0.740 &  0.917 &  0.877 \\
VAE~\cite{kingma_auto-encoding_2013-1}              &  0.997 &  0.999 &  0.936 &  0.959 &  0.973 &  0.964 &  0.993 &  0.976 &  0.923 &  0.976 &  0.970 \\
GAN~\cite{schlegl_unsupervised_2017}                &  0.926 &  0.995 &  0.805 &  0.818 &  0.823 &  0.803 &  0.890 &  0.898 &  0.817 &  0.887 &  0.866 \\
AnoGAN~\cite{schlegl_f-anogan_2019}                 &  0.966 &  0.992 &  0.850 &  0.887 &  0.894 &  0.883 &  0.947 &  0.935 &  0.849 &  0.924 &  0.913 \\
DSVDD~\cite{ruff_deep_2018}                         &  0.980 &  0.997 &  0.917 &  0.919 &  0.949 &  0.885 &  0.983 &  0.946 &  0.939 &  0.965 &  0.948 \\
AND~\cite{abati_latent_2019}                        &  0.993 &  0.999 &  0.959 &  0.966 &  0.956 &  0.964 &  0.994 &  0.980 &  0.953 &  0.981 &  0.975 \\

OCGAN~\cite{perera_ocgan_2019}                      &  0.998 &  0.999 &  0.942 &  0.963 &  0.975 &  \textbf{0.980} &  0.991 &  0.981 &  0.939 &  0.981 &  0.975 \\
\midrule
IF~\cite{liu_isolation-based_2012}                  &  0.969 &  0.995 &  0.751 &  0.837 &  0.876 &  0.752 &  0.874 &  0.906 &  0.737 &  0.883 &  0.858 \\
LOF~\cite{breunig_lof_2000}                         &  0.997 &  0.995 &  0.952 &  0.972 &  0.969 &  0.979 &  \textbf{0.998} &  0.977 &  0.917 &  0.976 &  0.973 \\
OCSVM~\cite{chen_one-class_2001}                    &  0.988 &  0.999 &  0.902 &  0.950 &  0.955 &  0.968 &  0.978 &  0.965 &  0.853 &  0.955 &  0.951 \\
KDE~\cite{bishop_pattern_2006}                      &  0.885 &  0.996 &  0.710 &  0.693 &  0.844 &  0.776 &  0.861 &  0.884 &  0.669 &  0.825 &  0.814 \\
LAD + LOF (ours) &  \textbf{0.999} &  0.999 &  \textbf{0.982} &  \textbf{0.983} &  0.975 &  0.974 &  0.996 &  0.981 &  \textbf{0.967} &  0.985 &  \textbf{0.984} \\
LAD + CAE (ours)                                    &  0.998 &  0.999 &  0.975 &  0.971 &  \textbf{0.981} &  0.976 &  0.995 &  \textbf{0.985} &  0.943 &  \textbf{0.990} &  0.981 \\ 
\bottomrule
\end{tabular}
}
\caption{Shows performance of existing anomaly detection methods on MNIST task using results from original papers if given split into network based (Top) and non-network based (Bottom).}
\label{tab:large_comparison}
\end{table*}

==> tables/large_comparison.tex <==
\begin{table*}
\scalebox{0.8}{
\begin{tabular}{lrrrrrrrrrr|r}
\toprule
 &      0 &      1 &      2 &      3 &      4 &      5 &      6 &      7 &      8 &      9 &   Mean \\
\midrule
LAD (ours)                &  0.984 &  0.992 &  0.920 &  0.917 &  0.921 &  0.871 &  0.971 &  0.942 &  0.928 &  0.945 &  0.939 \\
CAE                     &  0.996 &  0.999 &  0.946 &  0.940 &  0.971 &  0.945 &  0.992 &  0.979 &  0.901 &  0.985 &  0.965 \\
DCAE                     &  0.997 &  1.000 &  0.957 &  0.930 &  0.972 &  0.968 &  0.990 &  0.976 &  0.899 &  0.986 &  0.967 \\
RCAE~\cite{chalapathy_robust_2017}                     &  0.996 &  0.999 &  0.930 &  0.928 &  0.967 &  0.921 &  0.994 &  0.973 &  0.885 &  0.984 &  0.958 \\

DAE                      &  0.894 &  0.999 &  0.792 &  0.851 &  0.888 &  0.819 &  0.944 &  0.922 &  0.740 &  0.917 &  0.877 \\
VAE~\cite{kingma_auto-encoding_2013-1}                      &  0.997 &  0.999 &  0.936 &  0.959 &  0.973 &  0.964 &  0.993 &  0.976 &  0.923 &  0.976 &  0.970 \\
GAN~\cite{schlegl_unsupervised_2017}                      &  0.926 &  0.995 &  0.805 &  0.818 &  0.823 &  0.803 &  0.890 &  0.898 &  0.817 &  0.887 &  0.866 \\
AnoGAN~\cite{schlegl_f-anogan_2019}                   &  0.966 &  0.992 &  0.850 &  0.887 &  0.894 &  0.883 &  0.947 &  0.935 &  0.849 &  0.924 &  0.913 \\
DSVDD~\cite{ruff_deep_2018}                    &  0.980 &  0.997 &  0.917 &  0.919 &  0.949 &  0.885 &  0.983 &  0.946 &  0.939 &  0.965 &  0.948 \\
AND~\cite{abati_latent_2019}                      &  0.993 &  0.999 &  0.959 &  0.966 &  0.956 &  0.964 &  0.994 &  0.980 &  0.953 &  0.981 &  \textbf{0.975} \\
OCGAN~\cite{perera_ocgan_2019}                    &  0.998 &  0.999 &  0.942 &  0.963 &  0.975 &  0.980 &  0.991 &  0.981 &  0.939 &  0.981 &  \textbf{0.975} \\
\midrule
IF~\cite{liu_isolation-based_2012}        &  0.969 &  0.995 &  0.751 &  0.837 &  0.876 &  0.752 &  0.874 &  0.906 &  0.737 &  0.883 &  0.858 \\
LOF~\cite{breunig_lof_2000}                     &  0.997 &  0.995 &  0.952 &  0.972 &  0.969 &  0.979 &  0.998 &  0.977 &  0.917 &  0.976 &  \textbf{0.973} \\
OCSVM~\cite{chen_one-class_2001}                    &  0.988 &  0.999 &  0.902 &  0.950 &  0.955 &  0.968 &  0.978 &  0.965 &  0.853 &  0.955 &  0.951 \\
KDE~\cite{bishop_pattern_2006}                      &  0.885 &  0.996 &  0.710 &  0.693 &  0.844 &  0.776 &  0.861 &  0.884 &  0.669 &  0.825 &  0.814 \\
\bottomrule
\end{tabular}
}
\caption{Shows performance of existing anomaly detection methods on MNIST task using results from original papers if given split into network based (Top) and non-network based (Bottom).}
\label{tab:large_comparison}
\end{table*}


==> tables/mnist_corruption_table.tex <==
\begin{table*}
\centering
\scalebox{0.7}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Train Corrupt. &   0.00 &   0.01 &   0.02 &   0.03 &   0.04 &   0.05 &   0.06 &   0.07 &   0.08 &   0.09 &   0.10 \\
\midrule
LAD (ours) &  0.940 &  0.937 &  0.933 &  0.933 &  0.926 &  0.923 &  0.921 &  0.917 &  0.911 &  0.905 &  0.901 \\
LAD + CAE (ours) & \textbf{0.981} & \textbf{0.965} & \textbf{0.954} & \textbf{0.947} & \textbf{0.941} & \textbf{0.936} & \textbf{0.930} & \textbf{0.925} & \textbf{0.921} & \textbf{0.916} & \textbf{0.912} \\
ALOCC~\cite{sabokrou_adversarially_2018}      &  0.694 &  0.511 &  0.514 &  0.498 &  0.521 &  0.539 &  0.505 &  0.495 &  0.504 &  0.504 &  0.509 \\
CAE~\cite{hawkins_outlier_2002}        &  0.965 &  0.925 &  0.898 &  0.887 &  0.876 &  0.868 &  0.859 &  0.851 &  0.844 &  0.837 &  0.832 \\
DCAE~\cite{vincent_stacked_2010-1}       &  0.967 &  0.925 &  0.899 &  0.886 &  0.874 &  0.865 &  0.857 &  0.850 &  0.842 &  0.834 &  0.829 \\
DSVDD~\cite{ruff_deep_2018}      &  0.748 &  0.788 &  0.748 &  0.750 &  0.729 &  0.718 &  0.746 &  0.725 &  0.703 &  0.710 &  0.696 \\
IF~\cite{liu_isolation-based_2012} &  0.853 &  0.853 &  0.849 &  0.845 &  0.844 &  0.837 &  0.836 &  0.832 &  0.829 &  0.827 &  0.822 \\
LOF~\cite{breunig_lof_2000}              &  0.973 &  0.958 &  0.918 &  0.873 &  0.830 &  0.789 &  0.762 &  0.745 &  0.730 &  0.718 &  0.709 \\
OCSVM~\cite{scholkopf_estimating_2001}            &  0.954 &  0.895 &  0.867 &  0.853 &  0.840 &  0.828 &  0.819 &  0.812 &  0.806 &  0.800 &  0.794 \\
RCAE~\cite{chalapathy_robust_2017}                     &  0.957 &  0.934 &  0.906 &  0.894 &  0.881 &  0.870 &  0.861 &  0.854 &  0.845 &  0.838 &  0.832 \\
\bottomrule
\end{tabular}
}
\caption{Shows the mean AUC over digits over 3 seeds for training set corruption levels from 0\% to 10\% on MNIST. }
\vspace{-5mm}
\label{tab:mnist-corrupt}
\end{table*}
